The Goldilocks Principle: Reading Children's Books with Explicit Memory Representations

We introduce a new test of how well language models capture meaning in children's books. Unlike standard language modelling benchmarks, it distinguishes the task of predicting syntactic function words from that of predicting lower-frequency words, which carry greater semantic content. We compare a range of state-of-the-art models, each with a different way of encoding what has been previously read. We show that models which store explicit representations of long-term contexts outperform state-of-the-art neural language models at predicting semantic content words, although this advantage is not observed for syntactic function words. Interestingly, we find that the amount of text encoded in a single memory representation is highly influential to the performance: there is a sweet-spot, not too big and not too small, between single words and full sentences that allows the most meaningful information in a text to be effectively retained and recalled. Further, the attention over such window-based memories can be trained effectively through self-supervision. We then assess the generality of this principle by applying it to the CNN QA benchmark, which involves identifying named entities in paraphrased summaries of news articles, and achieve state-of-the-art performance.

==> Related.tex <==
\paragraph{Datasets}
There are clear parallels between the CBT and the Microsoft Research Sentence Completion Challenge (MSRCC) \citep{zweig2011microsoft}, which is also based on Project Gutenberg (but not children's books, specifically). The fundamental difference is that, where examples in the MSRCC are made of a single sentence, each query in the CBT comes with a wider context. This tests the sensitivity of language models to semantic coherence beyond sentence boundaries. The CBTest is also larger than the MRSCC (10,000 vs 1,040 test questions), requires models to select from more candidates on each question (10 vs 5), covers words of different (POS) types and contains large training and validation sets that match the form of the test set. 

There are also similarities between the CBT and the CNN/Daily Mail dataset recently released by \cite{nips15_hermann}.\footnote{The CNN/Daily Mail data is itself very similar to the the MCTest of machine comprehension \citep{richardson2013mctest}. However, the MCTest contains many fewer questions (\( \approx 700\)), which makes more susceptible to overfit solutions and less diagnostic of small model improvements.}  In this task, models must identify missing entities from bullet-point summaries of online news articles. All entities in both questions and stories are anonymized to prevent models from applying knowledge that cannot be inferred directly from the story. The CBT, in contrast, is intended as a more general test of the efficacy of language models, which might later be applied to generation, prediction or correction. Moreover, since the CBT does not contain anonymized entities, it incentivizes research into the integration of background knowledge (as well as the context and query) into models of language understanding. 

\paragraph{Models}
The idea of conditioning language models on some wider linguistic context is not new. Access to document-level features has been applied to improve both classical language models \cite{mikolov2012context} and word embeddings \cite{huang2012improving}. Unlike the present work, these studies did not explore different representation strategies for the wider context or their effect on interpreting and predicting specific word types.

The original Memory Network, introduced by \cite{weston2014memory} (with hard memory selection) was applied to question-answering tasks in which language was generated to describe the content of knowledge bases or simulated worlds. \cite{sukhbaatar2015end} and \cite{kumar2015ask} trained memory networks with RNN components end-to-end with soft memory access, and applied them to additional language tasks. The attention-based reading models of \cite{nips15_hermann} also have many commonalities with memory networks, the key difference being the absence of iterative access to the memory-like representations. Both \citep{kumar2015ask} and \citep{nips15_hermann} propose bidirectional RNNs as a way of representing previously read text. As mentioned previously, our findings in this work shed light on exactly why this is an effective strategy for semantically-focused language processing: bidirectional RNNs an learn to focus on small windows much like our convolutional window salient memory networks. 

Other recent papers have proposed RNN-like architectures with new ways of reading, storing and updating information to improve their capacity to learn algorithmic or syntactic patterns \citep{joulin2015inferring,dyer2015transition,grefenstette2015learning}. While we do not study these models in the present work, in future work the CBT can be used to test the applicability of these approaches to semantically-focused language modelling.



